ISIA-AF: Orchestrating Reproducible Attacks and Multi-Source Data Collection for OT Systems

Operational Technology (OT) environments require realistic, reproducible security datasets, yet existing approaches often lack automation, multi-source data capture, and sufficient documentation for reuse. This paper presents ISIA-AF, a modular attack framework for orchestrating reproducible attack execution and automated dataset generation on industrial systems. The framework coordinates distributed attack clients, records network traffic and operational data, ultimately leading to a multi-source dataset. We derive functional and non-functional requirements from prior work and stakeholder discussions, and realise the framework following a design science research approach. A case study on the ISIA testbed, comprising a real industrial system and a simulated process, demonstrates how the framework supports centralised control, low communication overhead, and flexible deployment across network segments. The result is a practical basis for generating extensible, multi-source OT security datasets for intrusion detection research.

==> packages.tex <==
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage[table]{xcolor}
\usepackage[utf8]{luainputenc}
\usepackage[british]{babel}
\usepackage[acronym, nomain]{glossaries}
\usepackage{marginnote}
\usepackage{tikz}
\usepackage{float}
\usepackage{tabularx}
\usepackage{booktabs}
\usepackage[backend=biber,style=ieee, mincitenames=1, maxcitenames=2, url=true, isbn=false, natbib]{biblatex}
\addbibresource[label=refs]{references.bib}
\usepackage{usebib}
\usepackage[hidelinks]{hyperref}
\usepackage[capitalise]{cleveref}
\usepackage{marginnote}
\usepackage{csquotes}

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

\AtEveryBibitem{%
	\ifentrytype{article}{%
		\clearfield{url}%
		\clearfield{urldate}%
	}{}%
	\ifentrytype{inproceedings}{%
		\clearfield{url}%
		\clearfield{urldate}%
	}{}%
}
\DeclareFieldFormat{urldate}{%
	\ifentrytype{article}{}{%
		\ifentrytype{inproceedings}{}{%
			\mkbibparens{\bibstring{urlseen}\space#1}%
		}%
	}%
}

\usetikzlibrary{patterns}

\bibinput{references}

\newbibfield{author}
\newbibfield{title}
\newbibfield{year}
\newcommand{\printarticle}[1]{\citeauthor{#1}, ``\usebibentry{#1}{title}''}
\newcommand{\printyear}[1]{\usebibentry{#1}{year}}
\newcommand{\fullc}{\tikz\fill[black] (0,0) circle (0.1cm);}
\newcommand{\quarc}{
	\tikz{
		\draw[black] (0,0) circle (0.1cm);
		\fill[black] (0,0) -- (0.1cm,0) arc [start angle=0, end angle=-90, radius=0.1cm] -- cycle;}}
\newcommand{\halfc}{\tikz{
		\draw[black] (0,0) circle (0.1cm);
		\fill[black] (0,0) -- (-0.1cm,0) arc [start angle=180, end angle=360, radius=0.1cm] -- cycle;}} 
\newcommand{\emptyc}{\tikz\draw[black] (0,0) circle (0.1cm);}

